Dark Sky Simulations: Early Data Release

The Dark Sky Simulations are an ongoing series of cosmological N-body simulations designed to provide a quantitative and accessible model of the evolution of the large-scale Universe. Such models are essential for many aspects of the study of dark matter and dark energy, since we lack a sufficiently accurate analytic model of non-linear gravitational clustering. In July 2014, we made available to the general community our early data release, consisting of over 55 Terabytes of simulation data products, including our largest simulation to date, which used $1.07 \times 10^{12}~(10240^3)$ particles in a volume $8h^{-1}\mathrm{Gpc}$ across. Our simulations were performed with 2HOT, a purely tree-based adaptive N-body method, running on 200,000 processors of the Titan supercomputer, with data analysis enabled by yt. We provide an overview of the derived halo catalogs, mass function, power spectra and light cone data. We show self-consistency in the mass function and mass power spectrum at the 1% level over a range of more than 1000 in particle mass. We also present a novel method to distribute and access very large datasets, based on an abstraction of the World Wide Web (WWW) as a file system, remote memory-mapped file access semantics, and a space-filling curve index. This method has been implemented for our data release, and provides a means to not only query stored results such as halo catalogs, but also to design and deploy new analysis techniques on large distributed datasets.

==> Makefile <==
DEPS = version.tex

mylatex=pdflatex -shell-escape
#mylatex=xelatex -shell-escape

all: ms.pdf

%.pdf: %.tex %.bbl $(DEPS)
	${mylatex} $(basename $<)
	${mylatex} $(basename $<)

%.bbl: %.tex
	${mylatex} $(basename $<)
	bibtex $(basename $<)

.PHONY: version.proto
version.proto:
	@echo `hg log -r . --template '{latesttag}-{latesttagdistance}-{node|short}\n'` > version.proto

version.tex: version.proto
	@cmp -s $< $@ || cp -p $< $@


==> VERSION.tex <==
0.1-36-5a1cb3393d63


==> tmp.tex <==
\subsection{A Brief Tour of the Dark Sky Simulations Early Data Release}

This material is intended to be useful to a wide audience, so it starts
at a very basic level. It ends at a very advanced level. Skip ahead if
you need to, or slow down and review the supplemental material.

First, you need to get the package with the basic data release. You can
use your web browser download feature to get a .zip or .tar.gz file.
They can be found at
\url{https://bitbucket.org/darkskysims/data_release/downloads} Or, if
you prefer the command line,

\begin{verbatim}
wget https://bitbucket.org/darkskysims/data_release/get/default.tar.gz
\end{verbatim}
The file you retrieve will be named something like
darkskysims-data\_release-dba678c57371.tar.gz and is currently about 4
Mbytes in size. You should unpack it.

\begin{verbatim}
tar xzf darkskysims-data_release-dba678c57371.tar.gz
cd darkskysims-data_release-dba678c57371/ds14_a
\end{verbatim}
If you are familiar with the mercurial version control system, and it is
installed on your system, you can replace the steps above with

\begin{verbatim}
hg clone https://bitbucket.org/darkskysims/data_release
cd data_release/ds14_a
\end{verbatim}
Using mercurial has additional advantages, since it can tell you if any
of the files have been changed or corrupted. Read more about mercurial
at \url{http://mercurial.selenic.com/}

Now let's look at some metadata,

\begin{verbatim}
head ds14_a_1.0000.head
\end{verbatim}
should produce the following output on a Unix-like operating system If
you don't have UNIX, use whatever tool is available to view an ASCII
file.

\begin{verbatim}
# SDF 1.0
int header_len =  2528;
parameter byteorder = 0x78563412;
int version = 2;
int version_2HOT = 2;
int units_2HOT = 2;
int64_t npart = 1073741824000;
float particle_mass = 5.6749434;
int iter = 543;
int do_periodic = 1;
\end{verbatim}
This is an SDF header. Our raw data is distributed in the SDF format.
The data\_release directory just contains the initial part (.head) of
this large file. Otherwise, you would need to wait to download the 34
Terabytes in the ds14\_a\_1.0000 file You can read more about SDF at
\url{http://bitbucket.org/JohnSalmon/sdf}. If you browse further down in
the file (perhaps using the more or less command) you will see,

\begin{verbatim}
double Omega0_m = 0.295037918703847;
double Omega0_lambda = 0.7048737821671822;
double Omega0_b = 0.04676431995034128;
double h_100 = 0.6880620000000001;
char length_unit[] = "kpc";
char mass_unit[] = "1e10 Msun";
char time_unit[] = "Gyr";
char velocity_unit[] = "kpc/Gyr";
char compiled_version_nln[] = "2HOT_nln-1.1.0-17-gbb2d669";
char compiled_date_nln[] = "Apr 19 2014";
char compiled_time_nln[] = "06:34:59";
\end{verbatim}
That is the metadata in the SDF file which describes the cosmological
parameters used, the physical units, and information describing the
exact version of the code. A bit further down is the first structure
declaration,

\begin{verbatim}
struct {
    unsigned int sha1_len;
    unsigned char sha1[20];
}[65536];
\end{verbatim}
This structure describes the layout in the data file of the sha1
checksums. There are 65536 of them, each with the length of data that
was checksummed and the sha1 checksum value. This allows one to verify
the integrity of each segment of the 34 Terabyte file independently.
Since the sha1 values are contained in the .head file in the
data\_release, their integrity can be verified with the checksum
contained within the mercurial repository. A change to any one of the
272 trillion bits in the data file can thereby be detected.

The main purpose of the SDF header is found in the last structure
definition,

\begin{verbatim}
struct {
    float x, y, z;              /* position of body */
    float vx, vy, vz;           /* velocity of body */
    int64_t ident;              /* unique identifier */
}[1073741824000];
\end{verbatim}
This tells us how to read the positions, velocities and identity of the
particles. There are 1073741824000 of them. Where are they? We tell you
in the .url file.

\begin{verbatim}
cat ds14_a_1.0000.url
http://darksky.slac.stanford.edu/simulations/ds14_a/ds14_a_1.0000
\end{verbatim}
The full 34 TB data file is on a machine at Stanford University. You
could download it like any of the millions of other files on the
Internet, but we have better ways.

If you like C and the command line, the SDF library is a good choice.
Check out the development version from our repository and compile it. It
will help for the next step if you have libcurl installed first.

\begin{verbatim}
cd ..
git clone http://bitbucket.org/darkskysims/sdf.git SDF
cd SDF
make
\end{verbatim}
This will build an executable called SDFcvt. It can be used to browse
SDF files. cp SDFcvt /usr/local/bin or elsewhere in your path if you
like. Change back to the ds14\_a subdirectory of the data\_release, and
try it out.

\begin{verbatim}
cd ../ds14_a
../SDF/SDFcvt ds14_a_1.0000.head Omega0_m Omega0_lambda Omega0_b h_100
0.29503791870384699 0.70487378216718222 0.046764319950341277 0.68806200000000006
\end{verbatim}
SDFcvt has parsed the cosmological values you specified from the header.
Now try this,

\begin{verbatim}
../SDF/SDFcvt -n 1 -s 1000000000000 http://dsdata.org/ds14_a_1.0000 x y z vx vy vz
3222417 3812104 2801807.5 -216.09906 -215.322311 273.964539
\end{verbatim}
That is the position and velocity of the trillionth particle in the data
file. -n 1 specifies that you want to read 1 element from the structure
-s specifies the offset in the array (Note that dsdata.org just
redirects to the Stanford web site listed above. Its purpose is to make
URLs shorter, so DarkSky names are easy to type, or fit on a line.)

If you see a message like this, you do not have libcurl installed

\begin{verbatim}
SFhdrio: MPMY_Fread returns -1, errno=22
\end{verbatim}
If you don't have libcurl, read on to see how you can use our python
library to access the data files over the Internet. You can also
download any of the smaller data files and use SDFcvt locally.

